You Shall Not Pass into Ring-0! A User Privacy-Friendly Anti-Cheat Architecture for Personal Computers

Kernel-level anti-cheats are effective against malicious player behavior in competitive video games, but raise significant user privacy concerns regarding installing unverifiable components at privileged modes (i.e., ring-0 in x86). While existing research has focused on improving the effectiveness of anti-cheats, the user privacy concern has been largely ignored. Tirith is an anti-cheat architecture that addresses this problem using two key ideas. First, instead of running video games within regular processes that players (as root admins) have control over, Tirith executes video games in Protected Virtual Machines that naturally sandbox computations from untrusted admins. Second, to monitor user behavior outside the sandbox (e.g., see if they are running malicious drivers), Tirith leverages a virtualization monitor that is trusted by both players and developers. Together, these ideas remove the need to run untrusted kernel-level anti-cheats, while providing the same level of protection compared to such solutions against a wide-range of common cheating mechanisms. The main challenge we face in implementing these ideas, however, is that the existing software stack for virtual machines is not designed to run video games and creates significant security and performance problems. We address these problems by proposing a security-focused Library OS kernel for games and an efficient graphics sharing pipeline for near-native rendering and display performance. In summary, without compromising on cheating behavior detection or performance, this work makes user privacy a first-class citizen in personal computers.

==> Makefile <==
MAIN ?= p
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
PPTX := $(patsubst pptx/%.pdf,fig/%-crop.pdf,$(wildcard pptx/*.pdf))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(PPTX) $(PLOT)
BTEX := --bibtex-args="-min-crossrefs=99"
LTEX := --latex-args="-interaction=nonstopmode -synctex=4"
SHELL:= $(shell echo $$SHELL)
APP  := appendix.tex

all: $(DEPS) ## generate a pdf
	@TEXINPUTS="sty:" python3 bin/latexrun.py $(BTEX) $(LTEX) $(MAIN)
	cp latex.out/p.synctex.gz p.synctex.gz

appendix.pdf: appendix-new.tex
	pdflatex $^
	bibtex appendix-new
	bibtex appendix-new
	bibtex appendix-new
	bibtex appendix-new

submit: $(DEPS) ## proposal function
	@bin/nsf-submit.py $(MAIN).pdf $(CURDIR)/nsf-submit

diff: $(DEPS) ## generate diff-highlighed pdf
	@bin/diff.sh $(DIFF)

help: ## print help
	@grep -E '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
		| sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-10s\033[0m %s\n", $$1, $$2}'

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
		 "$(shell git rev-parse --short HEAD)"            \
		 "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/% ## build highlighted tex code from source code
	pygmentize -P tabsize=4 -P mathescape -f latex $^ | python3 bin/mark.py > $@

code/fmt.tex: ## generate color table
	pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg ## generate pdf from svg
	inkscape --without-gui -f $^ -D -A $@

fig/%-crop.pdf: pptx/%.pdf
	pdfcrop --margin=1 $^ $@

data/%.tex: data/%.gp ## generate plot
	gnuplot $^

draft: $(DEPS) ## generate pdf with a draft info
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" python3 bin/latexrun.py $(BTEX) $(MAIN)

watermark: $(DEPS) ## generate pdf with a watermark
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" python3 bin/latexrun.py $(BTEX) $(MAIN)

spell: ## run a spell check
	@for i in *.tex; do bin/aspell.sh $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex
	@pdftotext $(MAIN).pdf /dev/stdout | grep '??'

spell2:
	@ for i in *.tex latex.out/*.bbl; do aspell -t $(ASPELL_CMDS) -p ./aspell.words -c $$i; done
	@ ( head -1 aspell.words ; tail -n +2 aspell.words | LC_ALL=C sort ) > aspell.words~
	@ mv aspell.words~ aspell.words

.PHONY: spell


clean: ## clean up
	@python3 bin/latexrun.py --clean
	rm -f abstract.txt
	rm -f p.synctex.gz

distclean: clean ## clean up completely
	rm -f code/*.tex

init: ## init writing (discarding example)
	rm -f {code,fig,data}/ex-*
	perl -pi -e 's/^\\input{ex}/% \\input{ex}/g' $(MAIN).tex

abstract.txt: abstract.tex $(MAIN).tex ## generate abstract.txt
	@python3 bin/mkabstract.py $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init


==> README <==
die: a paper template
=====================

## start
0. Prerequisites
  - Python 3.x

  - pygmentize

    $ pip install Pygments 

1. clone the git repo:

  - if you have none,

    $ git clone --depth=1 git@github.com:tsgates/die.git

  - if you have a git-repo to work on,

    $ git subtree add --squash git@github.com:tsgates/die.git master -P paper

2. build it:

    $ make
    p.pdf built @Tue May 20 20:38:19 EDT 2014
    
    (check p.pdf)

3. starting point, p.tex:

    $ grep -oP 'input{\K\w+' p.tex
    cmds
    rev
   *hdr
    abstract
   *ex
    intro
    overview
    design
    impl
    eval
    conclusion
    ack

  - hdr: includes title/author info
  - ex : includes latex examples

4. example latex

    $ git checkout example
    $ make

5. formatting rules (dependencies)

  - code/*.{c,cc,py,js ...} -> code/*.tex
  - fig/*.svg               -> fig/*.pdf
  - data/*.gp               -> fig/*.tex

  (see ex.tex for more details)

## tools

1. make a draft for revision

    $ make draft
    $ make watermark

2. abstract.txt (from abstract.tex)

    $ cat abstract.txt 

3. highlight changes, since the last submit

    $ make diff DIFF=HEAD@{}

4. spell check

    $ make spell



==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}

We would like to thank the anonymous reviewers and our shepherd, Bryan Parno, for their insightful reviews which significantly improved the paper's evaluation and presentation.
% 
This work was partly supported by the National Science Foundation (NSF)  under grants CNS-2145888 and the National Research Foundation of Korea (NRF) grant funded by the Korea government (MSIT) (No. RS-2023-00209093).

==> code/enclave-signing-oracle.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{let} \PY{n+nf}{enclaveSigningOracle}\PY{p}{(}\PY{n+nl}{attestationPrivateKeySGX}\PY{p}{:} \PY{n}{skey}\PY{p}{,}
                         \PY{n+nl}{overlordMachineID}\PY{p}{:} \PY{n}{bitstring}\PY{p}{)} \PY{o}{=}
  \PY{n}{in}\PY{p}{(}\PY{n}{enclave\PYZus{}signing\PYZus{}chan}\PY{p}{,} \PY{p}{(}\PY{n+nl}{nonce}\PY{p}{:} \PY{n}{bitstring}\PY{p}{,}
          \PY{n+nl}{machineID}\PY{p}{:} \PY{n}{bitstring}\PY{p}{,} \PY{n+nl}{sgxdig}\PY{p}{:}\PY{n}{sgxDigest}\PY{p}{)}\PY{p}{)}\PY{p}{;}
  \PY{k}{if} \PY{n}{machineID} \PY{o}{=} \PY{n}{overlordMachineID} \PY{n}{then}
    \PY{k}{if} \PY{n}{sgxdig} \PY{o}{=} \PY{n}{correctSGXDigest} \PY{n}{then} \PY{l+m+mi}{0}
    \PY{k}{else}
      \PY{n}{out}\PY{p}{(}\PY{n}{enclave\PYZus{}signing\PYZus{}chan}\PY{p}{,} \PY{n}{sign}\PY{p}{(}\PY{p}{(}\PY{n}{nonce}\PY{p}{,} \PY{n}{machineID}\PY{p}{,} \PY{n}{sgxdig}\PY{p}{)}\PY{p}{,}
                                  \PY{n}{attestationPrivateKeySGX}\PY{p}{)}\PY{p}{)}
  \PY{k}{else}
    \PY{n}{out}\PY{p}{(}\PY{n}{enclave\PYZus{}signing\PYZus{}chan}\PY{p}{,}
      \PY{n}{sign}\PY{p}{(}\PY{p}{(}\PY{n}{nonce}\PY{p}{,} \PY{n}{machineID}\PY{p}{,} \PY{n}{sgxdig}\PY{p}{)}\PY{p}{,} \PY{n}{attestationPrivateKeySGX}\PY{p}{)}\PY{p}{)}\PY{p}{.}
\end{Verbatim}


==> code/fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/inst-call.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{call} \PY{n+nv}{function\PYZus{}addr}  

\PY{c+c1}{; After}
  \PY{n+nf}{sub} \PY{n+nv}{R13}\PY{p}{,} \PY{l+m+mi}{8}                \PY{c+c1}{; Adjust original stack top address}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{R13}              \PY{c+c1}{; Pass original address to R15}
  \PY{n+nf}{call} \PY{n+nv}{data\PYZus{}translator}      \PY{c+c1}{; Translate to new address}
  \PY{n+nf}{mov} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{),} \PY{n+nv}{return\PYZus{}addr}    \PY{c+c1}{; save the original return\PYZus{}addr at R15}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{function\PYZus{}addr}    \PY{c+c1}{; Pass original function address}
  \PY{n+nf}{call} \PY{n+nv}{code\PYZus{}translator}      \PY{c+c1}{; Translate the original function address}
                            \PY{c+c1}{; to shuffled function address}
\PY{n+nl}{return\PYZus{}addr:}
  \PY{n+nf}{jmp} \PY{o}{*}\PY{n+nv}{R14}                  \PY{c+c1}{; jump to the shuffled function address}
\end{Verbatim}


==> code/inst-return.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{return}

\PY{c+c1}{; After}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{R13}                \PY{c+c1}{; Pass the stack top address }
  \PY{n+nf}{call} \PY{n+nv}{data\PYZus{}translator}        \PY{c+c1}{; Translate original stack top}
                              \PY{c+c1}{; address to shuffled stack top address }
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{)}              \PY{c+c1}{; Restore original return address from}
                              \PY{c+c1}{; the shuffled stack top address}
  \PY{n+nf}{call} \PY{n+nv}{code\PYZus{}translator}        \PY{c+c1}{; Translate original return address to}
                              \PY{c+c1}{; shuffled return address}
  \PY{n+nf}{add} \PY{n+nv}{R13}\PY{p}{,} \PY{l+m+mi}{8}                  \PY{c+c1}{; Adjust the stack pointer}
  \PY{n+nf}{jmp} \PY{o}{*}\PY{n+nv}{R14}                    \PY{c+c1}{; then, jump to the shuffled return address}
\end{Verbatim}


==> code/inst-store.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{mov} \PY{l+m+mi}{4}\PY{p}{(}\PY{n+nb}{RAX}\PY{p}{),} \PY{n+nb}{RBX}           \PY{c+c1}{; Store RBX at (RAX + 4)}

\PY{c+c1}{; After}
  \PY{n+nf}{lea} \PY{n+nv}{R15}\PY{p}{,} \PY{l+m+mi}{4}\PY{p}{(}\PY{n+nb}{RAX}\PY{p}{)}           \PY{c+c1}{; Pass the original address using R15}
  \PY{n+nf}{call} \PY{n+nv}{data\PYZus{}translator}      \PY{c+c1}{; data\PYZus{}translator searches T\PYZhy{}TABLE}
                            \PY{c+c1}{; and returns new address using R15}
  \PY{n+nf}{mov} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{),} \PY{n+nb}{RBX}            \PY{c+c1}{; Write a value RBX to R15}
\end{Verbatim}


==> code/pht.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n+nl}{force\PYZus{}pht\PYZus{}state:}
\PY{n+nf}{cmp} \PY{o}{\PYZpc{}}\PY{n+nb}{rcx}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nb}{rcx}
\PY{n+nf}{je} \PY{n+nv}{.L0}\PY{c+c1}{; nop; je .L1; nop; ......; je .L16384; nop;}
\end{Verbatim}


==> code/policy-mbedtls.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{// Developer specified policy}

\PY{k}{static} \PY{k+kt}{void} \PY{n+nf}{mbedtls\PYZus{}mpi\PYZus{}montmul}\PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{)} \PY{n}{\PYZus{}\PYZus{}attribute\PYZus{}\PYZus{}}\PY{p}{(}\PY{p}{(}\PY{n}{randomize}\PY{p}{)}\PY{p}{)}\PY{p}{;}
\PY{k}{static} \PY{k+kt}{void} \PY{n+nf}{rsa\PYZus{}decrypt}\PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{)} \PY{p}{\PYZob{}}

\PY{k}{do} \PY{p}{\PYZob{}}
\PY{c+c1}{// sensitive branch conditions}
\PY{k}{if} \PY{p}{(}\PY{n}{bit} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{1}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{c+c1}{// shuffling event}
  \PY{n}{mbedtls\PYZus{}mpi\PYZus{}montmul}\PY{p}{(}\PY{p}{)}\PY{p}{;}
  \PY{c+c1}{// shuffling event}
  \PY{n}{mbedtls\PYZus{}mpi\PYZus{}montmul}\PY{p}{(}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{k}{else} \PY{p}{\PYZob{}}
  \PY{c+c1}{// shuffling event}
  \PY{n}{mbedtls\PYZus{}mpi\PYZus{}montmu}\PY{p}{(}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}
\PY{k}{while} \PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{)}\PY{p}{;}
\PY{c+c1}{// rest of the code}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/policy1.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{// Insecure shuffling policy}

\PY{c+c1}{// randomization event (T)}
\PY{n}{\PYZus{}\PYZus{}randomize}\PY{p}{(}\PY{p}{)}\PY{p}{;}

\PY{c+c1}{// sensitive branch conditions}
\PY{k}{do} \PY{p}{\PYZob{}}

\PY{k}{if} \PY{p}{(}\PY{n}{bit} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{1}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{n}{func\PYZus{}one}\PY{p}{(}\PY{p}{)}\PY{p}{;}
  \PY{n}{func\PYZus{}two}\PY{p}{(}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{k}{else} \PY{p}{\PYZob{}}
  \PY{n}{func\PYZus{}one}\PY{p}{(}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k}{while} \PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{)}

\PY{c+c1}{// randomization event (T+1)}
\PY{n}{\PYZus{}\PYZus{}randomize}\PY{p}{(}\PY{p}{)}\PY{p}{;}
\end{Verbatim}


==> code/queries-copy.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{p}{(}\PY{o}{*}
  \PY{n}{Query} \PY{err}{\PYZsh{}}\PY{l+m+mf}{1.} \PY{n}{Locality} \PY{n}{test} \PY{n}{should} \PY{n}{complete} \PY{n}{successfully}\PY{p}{.}
$\star$\PY{p}{)}
\PY{n}{query} \PY{n+nl}{tok}\PY{p}{:}\PY{n}{bitstring}\PY{p}{,} \PY{n+nl}{encMeasure}\PY{p}{:} \PY{n}{sgxDigest}\PY{p}{;}
  \PY{n}{event}\PY{p}{(}\PY{n}{LocalityTestPassed}\PY{p}{(}\PY{n}{tok}\PY{p}{,} \PY{n}{encMeasure}\PY{p}{)}\PY{p}{)}\PY{p}{.}

\PY{p}{(}\PY{o}{*} \PY{n}{Query} \PY{err}{\PYZsh{}}\PY{l+m+mf}{2.} \PY{n}{Locality} \PY{n}{test} \PY{n}{should} \PY{n}{only} \PY{n}{succeed} \PY{n}{after} \PY{n}{these}
   \PY{n}{events} \PY{n}{occur} \PY{n}{in} \PY{n}{order}\PY{p}{.} \PY{o}{*}\PY{p}{)}
\PY{n}{query} \PY{n+nl}{tok}\PY{p}{:} \PY{n}{bitstring}\PY{p}{,} \PY{n+nl}{encMeasure}\PY{p}{:} \PY{n}{sgxDigest}\PY{p}{,}
                      \PY{n+nl}{mID}\PY{p}{:} \PY{n}{machineIdentifier}\PY{p}{;}
  \PY{n}{event}\PY{p}{(}\PY{n}{LocalityTestPassed}\PY{p}{(}\PY{n}{tok}\PY{p}{,} \PY{n}{encMeasure}\PY{p}{)}\PY{p}{)}     \PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}
  \PY{p}{(}\PY{n}{event}\PY{p}{(}\PY{n}{ResponseSentFromOverlord}\PY{p}{(}\PY{n}{tok}\PY{p}{,} \PY{n}{encMeasure}\PY{p}{)}\PY{p}{)} \PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}
  \PY{p}{(}\PY{n}{event}\PY{p}{(}\PY{n}{TokenReceivedbyOverlord}\PY{p}{(}\PY{n}{tok}\PY{p}{,} \PY{n}{mID}\PY{p}{)}\PY{p}{)} \PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}
  \PY{p}{(}\PY{n}{event}\PY{p}{(}\PY{n}{TokenReceivedbyEnclave}\PY{p}{(}\PY{n}{tok}\PY{p}{,} \PY{n}{mID}\PY{p}{)}\PY{p}{)} \PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}
  \PY{p}{(}\PY{n}{event}\PY{p}{(}\PY{n}{TokenSentfromUser}\PY{p}{(}\PY{n}{tok}\PY{p}{)}\PY{p}{)} \PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}
  \PY{p}{(}\PY{n}{event}\PY{p}{(}\PY{n}{LocalityTestInitiated}\PY{p}{(}\PY{n}{tok}\PY{p}{,} \PY{n}{encMeasure}\PY{p}{)}\PY{p}{)}
  \PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{.}
\end{Verbatim}


==> code/queries.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{p}{(}\PY{o}{*} \PY{n}{SQ}\PY{p}{.} \PY{n}{ColocationCheckPassed} \PY{n}{should} \PY{n}{be} \PY{n}{triggered} \PY{k}{if} \PY{n}{machine}
   \PY{n}{X} \PY{n}{and} \PY{n}{Y} \PY{n}{are} \PY{n}{the} \PY{n}{same} \PY{n}{and} \PY{n}{the} \PY{n}{enclaves} \PY{n}{are} \PY{n}{the} \PY{n}{same}\PY{p}{.} \PY{o}{*}\PY{p}{)}
\PY{n}{query} \PY{n+nl}{Tok}\PY{p}{:}\PY{n}{token}\PY{p}{,}\PY{n+nl}{EncX}\PY{p}{:} \PY{n}{sgxDigest}\PY{p}{,} \PY{n+nl}{EncY}\PY{p}{:}\PY{n}{sgxDigest}\PY{p}{,} 
                  \PY{n+nl}{LocX}\PY{p}{:} \PY{n}{machine}\PY{p}{,} \PY{n+nl}{LocY}\PY{p}{:} \PY{n}{machine}\PY{p}{;}
  \PY{n}{event}\PY{p}{(}\PY{n}{ColocationCheckPassed}\PY{p}{(}\PY{n}{Tok}\PY{p}{,} \PY{n}{EncX}\PY{p}{)}\PY{p}{)}             \PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}
    \PY{n}{event}\PY{p}{(}\PY{n}{OverlordExistsAtLocation}\PY{p}{(}\PY{n}{LocX}\PY{p}{)}\PY{p}{)}            \PY{o}{\PYZam{}}\PY{o}{\PYZam{}}
    \PY{n}{event}\PY{p}{(}\PY{n}{EnclaveExistsAtLocation}\PY{p}{(}\PY{n}{LocY}\PY{p}{,} \PY{n}{EncY}\PY{p}{)}\PY{p}{)}       \PY{o}{\PYZam{}}\PY{o}{\PYZam{}}
    \PY{n}{LocX} \PY{o}{=} \PY{n}{LocY} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{n}{EncX} \PY{o}{=} \PY{n}{EncY}\PY{p}{.}

\PY{p}{(}\PY{o}{*} \PY{n}{RQ}\PY{p}{.} \PY{n}{ColocationCheckPassed} \PY{n}{should} \PY{n}{be} \PY{n}{triggered}\PY{p}{.} \PY{o}{*}\PY{p}{)}
\PY{n}{query} \PY{n+nl}{Tok}\PY{p}{:}\PY{n}{token}\PY{p}{,} \PY{n+nl}{Enc}\PY{p}{:} \PY{n}{sgxDigest}\PY{p}{;}
  \PY{n}{event}\PY{p}{(}\PY{n}{ColocationCheckPassed}\PY{p}{(}\PY{n}{Tok}\PY{p}{,} \PY{n}{Enc}\PY{p}{)}\PY{p}{)}
\end{Verbatim}


==> code/read-attack.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cm}{/* Sample data attack */}

\PY{c+cm}{/* enclave.edl */}
\PY{k+kt}{size\PYZus{}t} \PY{n+nf}{ocall\PYZus{}read}\PY{p}{(}\PY{k+kt}{int} \PY{n}{fd}\PY{p}{,} \PY{p}{[}\PY{n}{user\PYZus{}check}\PY{p}{]} \PY{k+kt}{char}\PY{o}{*} \PY{n}{buf}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{n}{len}\PY{p}{)}\PY{p}{;}

\PY{c+cm}{/* main.cpp */}
\PY{k+kt}{void} \PY{n+nf}{sensitive\PYZus{}function}\PY{p}{(}\PY{p}{)} \PY{p}{\PYZob{}}

  \PY{k+kt}{char} \PY{n}{buf}\PY{p}{[}\PY{l+m+mi}{100}\PY{p}{]}\PY{p}{;}
  \PY{k+kt}{int} \PY{n}{allowed} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;}

  \PY{c+c1}{// if len = 101, it will overflow}
  \PY{n}{ret\PYZus{}len} \PY{o}{=} \PY{n}{ocall\PYZus{}read}\PY{p}{(}\PY{n}{fd}\PY{p}{,} \PY{n}{buf}\PY{p}{,} \PY{n}{len}\PY{p}{)}\PY{p}{;}

  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/senc.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{p}{(}\PY{o}{*} \PY{n}{Abstract} \PY{n}{types} \PY{o}{*}\PY{p}{)}

\PY{n}{type} \PY{n}{key}\PY{p}{.} \PY{n}{type} \PY{n}{message}\PY{p}{.}

\PY{p}{(}\PY{o}{*} \PY{n}{Encryption}\PY{o}{/}\PY{n}{decryption} \PY{n}{routines}\PY{o}{*}\PY{p}{)}

\PY{n}{fun} \PY{n}{senc}\PY{p}{(}\PY{n}{message}\PY{p}{,}\PY{n}{key}\PY{p}{)}\PY{o}{:} \PY{n}{message}\PY{p}{.}     \PY{p}{(}\PY{o}{*} \PY{n}{symmetric} \PY{n}{encryption} \PY{o}{*}\PY{p}{)}

\PY{n}{reduc} \PY{n}{forall} \PY{n+nl}{m}\PY{p}{:} \PY{n}{message}\PY{p}{,} \PY{n+nl}{k}\PY{p}{:} \PY{n}{key}\PY{p}{;}
  \PY{n}{sdec}\PY{p}{(}\PY{n}{senc}\PY{p}{(}\PY{n}{m}\PY{p}{,} \PY{n}{k}\PY{p}{)}\PY{p}{,} \PY{n}{k}\PY{p}{)} \PY{o}{=} \PY{n}{m}\PY{p}{.}          \PY{p}{(}\PY{o}{*} \PY{n}{symmetric} \PY{n}{decryption} \PY{o}{*}\PY{p}{)}
\end{Verbatim}


==> code/sgx-shield.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{load} \PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{)} \PY{p}{\PYZob{}}

\PY{c+c1}{// Rest of the code}

\PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}value} \PY{o}{=} \PY{p}{(}\PY{n}{Elf64\PYZus{}Addr}\PY{p}{)}
  \PY{n}{reserve}\PY{p}{(}\PY{n}{pshdr}\PY{p}{[}\PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}shndx}\PY{p}{]}\PY{p}{.}\PY{n}{sh\PYZus{}flags}\PY{p}{,}
    \PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}size}\PY{p}{,} \PY{n}{pshdr}\PY{p}{[}\PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}shndx}\PY{p}{]}\PY{p}{.}\PY{n}{sh\PYZus{}addralign}\PY{p}{)}\PY{p}{;}

\PY{c+cm}{/* fill zeros for .bss section .. otherwise, copy from file */}
\PY{k}{if} \PY{p}{(}\PY{n}{pshdr}\PY{p}{[}\PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}shndx}\PY{p}{]}\PY{p}{.}\PY{n}{sh\PYZus{}type} \PY{o}{=}\PY{o}{=} \PY{n}{SHT\PYZus{}NOBITS}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{n}{fill\PYZus{}zero}\PY{p}{(}\PY{p}{(}\PY{k+kt}{char} \PY{o}{*}\PY{p}{)}\PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}value}\PY{p}{,} \PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}size}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{k}{else} \PY{p}{\PYZob{}}
  \PY{n}{cpy}\PY{p}{(}\PY{p}{(}\PY{k+kt}{char} \PY{o}{*}\PY{p}{)}\PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}value}\PY{p}{,} \PY{n}{GET\PYZus{}OBJ}\PY{p}{(}\PY{k+kt}{char}\PY{p}{,} \PY{n}{symoff}\PY{p}{)}\PY{p}{,}
    \PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}size}\PY{p}{)}\PY{p}{;}

  \PY{c+cm}{/* update last values */}
  \PY{n}{last\PYZus{}size} \PY{o}{=} \PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}size}\PY{p}{;}
  \PY{n}{last\PYZus{}off} \PY{o}{=} \PY{n}{symoff}\PY{p}{;}
  \PY{n}{last\PYZus{}st\PYZus{}value} \PY{o}{=} \PY{n}{symtab}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{st\PYZus{}value}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{c+c1}{// Rest of the code}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> rev.tex <==
\gdef\therev{7e6dbcb}
\gdef\thedate{2026-04-17 16:52:06 +0800}


==> tables/comparison.tex <==
{
% \setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lcl|c|c@{}}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}System \\ property\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{System software environment}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Enclave-based \\ environment\\ {[}{]}\end{tabular}}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VBSG\\ {[}this work{]}\end{tabular}} \\ \cmidrule(lr){2-3}
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Kernel modules\\ {[EVC,Vanguard...]}\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Distributed VMM \\ logging {[AVM]}\end{tabular}} &  &  \\
\multicolumn{1}{c}{} & \multicolumn{1}{l}{} &  &  &  \\ \midrule
\multicolumn{2}{l}{\textbf{Protection capability}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
Anti-cheating & -- & \multicolumn{1}{c|}{Yes} & Yes & Yes \\
Memory hack & -- & \multicolumn{1}{c|}{No} & No & Yes \\
Digital rights & -- & \multicolumn{1}{c|}{No} & No & Yes \\
\multicolumn{2}{l}{\textbf{Trust isolation boundary}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
 System privilege & \multicolumn{2}{c|}{Full client system} & Enclave & Game VM \\
 Protected device & NA & \multicolumn{1}{c|}{NA} & NA & Input device \\
\textbf{Trust requirement} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
Game developer & Trust client OS & \multicolumn{1}{c|}{No require.} & No require. & No require. \\
Client player & \multicolumn{2}{c|}{Trust game protection software} & No require. & No require. \\
\multicolumn{2}{l}{\textbf{Deployment scalability}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
Perf. overhead & Low & \multicolumn{1}{c|}{Low} & Med & Low \\
Modification & Low & \multicolumn{1}{c|}{Low} & Med & Low \\
Platform & All & \multicolumn{1}{c|}{All} & Intel & All \\ \bottomrule
\end{tabular}
}


==> tables/implementation.tex <==
\begin{tabular} {ll@{~~}lrl@{~~}lr}
\toprule
  \textbf{Component}  & \textbf{Base} & \textbf{Ver.} & \textbf{SLoC} \\
\midrule
{\bf Library OS Kernel} \\

  ~~ Additional system calls           & Gramine &  v1.7     & $2k$   \\
  % \sysmonitor           & Erebor~\cite{erebor} &  v1.7     & $550$   \\
   ~~PAL Layer       & Gramine &  v1.7     & $700$   \\
  ~~Render/display libraries          & -- &  --     & $3k$   \\
\midrule
  {\bf QEMU VMM} \\
  % & Linux/KVM & 5.16.9 & 573 \\
  % \systrim          & OP-TEE~\cite{optee} & 3.10.0 & $158$   
  % \\
  % & Linux kernel & 5.16.9 & 274    \\
  ~~tirith-listener & QEMU & v10.1.50 & $1k$  \\
\bottomrule 
\end{tabular}


==> threat_model.tex <==
\section{Threat Model}
\label{s:threatModel}

% We assume 

==> tying.tex <==
\subsection{Tying Up with Our Guiding Principles}

\label{sec:des:guide}
%
After presenting the design of \sys along with its protection schemes,
we show how \sys ties up perfectly with our guiding principles (mentioned
in \AD{XXX}).


\sys's framework is designed to directly comply with the first guiding principle
(illustrated as $P1$ in~\autoref{sec:motivation:guiding}).
%
In particular, we do not consider a specific set of side-channel attacks while
designing of our scheme.
%
Instead, we provide an overarching framework, devised after understanding
the different ways shared resources are exploited to launch attacks against SGX
enclaves.
%
Then, we devise a methodology for protecting shared resources using \sys's framework
and extend it to protect against all demonstrated side-channels in Intel SGX.
%
We discuss how \sys's framework and protection methodology can be used to defend
extend \sys's protections to future side-channels in \AD{XXX}.

%
Furthermore, the current protection schemes (mentioned in \AD{XXX}) directly
comply with $P2$, i.e., no enclave-related secret unknown to the attacker is
stored by \sys.
%
This ensures that our implementation is resistant to side-channels and an
unlikely takeover of the system will only reduce the enclave to its original
protections.
%
As a direct consequence of our lightweight protection schemes, \sys's TCB is
minimal, i.e., only 7K LoC which complies with $P3$ of our guiding principle.
%\subsection{Compliance with P4}
%
Lastly, \sys also complies with $P4$, i.e., our scheme induces an overhead of
$30.4\%$ on micro-benchmarks and an overhead of \AD{XXX} on real-world applications.
%
% Furthermore, our scheme improves on the next-best scheme~\cite{raccoon} by more than an
% order of magnitude.

\AD{Not sure if this is the right position or we even need this "tying with our
guiding principles section"}


==> warning.tex <==
\usepackage{silence}
\WarningFilter*{caption}{Unsupported document class}
